Frontier models need only one text to unmask its human or AI author

Given a single text and a simple zero-shot prompt (no web access, tools, candidate lists, or writing samples), frontier models can answer "who wrote this?" at three increasingly specific levels: (1) whether an AI or human wrote it, (2) if an AI, which lab, and (3) if a human, often exactly who. The latest models (Claude Fable 5.2, GPT-6.1 Sol, Gemini 4 Carbon) match trained detectors like Pangram while also explaining their predictions in natural language, and Opus 5.5 names the correct lab for 98% of texts generated by models from Anthropic, OpenAI, and Google. Most strikingly, Fable 5.2 correctly names the author of 55% of 15K anonymous ICML 2020 reviews that were never made public, and identifies the username behind 69% of comments from active Redditors (with >500 posts over the last year). Accuracy depends on exposure to an author's writing in pretraining data and on reasoning effort, and simply asking a model how familiar it is with someone predicts whether it can identify their writing. For anyone who has published enough writing online, frontier models present a greater threat to anonymity than commonly assumed, and defenses are limited.

==> labels/archive_labels.tex <==
\makeatletter
\providecommand{\externallabel}[2]{\AtBeginDocument{\@ifundefined{r@#1}{\global\@namedef{r@#1}{#2}}{}}}
\externallabel{app:limitations}{{A}{1}{}{appendix.A}{}}
\externallabel{app:robustness_all}{{B}{1}{}{appendix.B}{}}
\externallabel{tab:deniz-agent:length-accuracy}{{1}{2}{\textbf {Length and verdict accuracy.} All six rows use the same 38,541 documents. \model {} reads the outline and \twinmodel {} the document; both use their saved global verdicts at the calibrated 1\% false-positive-rate cut. Opus and Sol use their joint-prompt verdicts ($\mathrm {ai\_share}\geq 0.5$). The partial Pearson $r$ relates $\log _2$ whitespace word count to binary correctness after removing means within dataset $\times $ condition $\times $ provenance quadrant (70 groups). The slope gives the associated percentage-point change in accuracy per doubling of length. Two-sided $p$-values use evaluation-cluster CR1 uncertainty (22 clusters, $t_{21}$ reference), with Holm correction across six tests. Bold $p$-values are below 0.05. These are exploratory linear associations, not causal effects; whitespace counts are not comparable across all languages}{table.caption.2}{}}
\externallabel{tab:deniz-agent:genre-accuracy}{{2}{2}{\textbf {Fiction versus nonfiction verdict accuracy within provenance quadrants.} Source-defined genre labels identify 4,203 fiction and 22,911 nonfiction documents from the same shared detector population. Cells give the fiction-minus-nonfiction accuracy difference in percentage points; parentheses give the evaluation-cluster CR1 $p$-value after Holm correction across all 18 comparisons. Positive differences favor fiction. Datasets and conditions are pooled within each quadrant; length is excluded. Detector verdict rules match Table~\ref {tab:deniz-agent:length-accuracy}. Q1 is human ideas/human prose; Q3 is model ideas/model prose; Q4 is human ideas/model prose. Fiction/nonfiction counts are 1,194/7,270 in Q1, 2,571/8,451 in Q3, and 388/7,190 in Q4. Q2 has 50 fiction documents and no nonfiction comparator. Cluster counts are 14, 13 and 9, respectively; Q4 fiction spans only two evaluations. Thus inference is approximate and differences remain confounded with dataset and condition composition}{table.caption.3}{}}
\externallabel{app:atrey_rq1_timeline}{{C}{2}{}{appendix.C}{}}
\externallabel{app:atrey_rq1_full}{{D}{3}{}{appendix.D}{}}
\externallabel{tab:atrey_rq1_full}{{4}{4}{RQ1 on the full corpus, matched across the ten judges; Gemini~4 Carbon is scored on the same documents}{table.caption.4}{}}
\externallabel{tab:atrey_rq1_operating}{{5}{4}{Frontier models have few false positives, where a fully human document is misclassified as AI. Recall is defined as the share of AI text flagged as AI (in \%). For prompted models, we classify a document as AI if its reported AI share is at least 0.5. For trained detectors, we use their pre-existing cutoffs. @1\% is the recall such that the FPR is at or below 1\%}{table.caption.5}{}}
\externallabel{fig:atrey_rq1_cost}{{1}{5}{Accuracy against cost on the matched corpus (standard API prices, estimates). Aubergine points and the line mark the cost frontier. On Q4, Sol is the cheapest detector near 80\%}{figure.caption.6}{}}
\externallabel{fig:atrey_rq1_reliability}{{2}{5}{Stated \texttt {ai\_share} against the share of documents that are AI, by score bin. Bins under 30 documents are left out. Curves above the diagonal mean a score understates how often the text is AI-generated in this corpus; the corpus is mostly AI-generated, so this reflects the corpus mix as well as the judge}{figure.caption.7}{}}
\externallabel{fig:atrey_rq1_capability}{{3}{5}{Detection tracks general capability: balanced both-correct accuracy (Bal., \%) on the 1,000-document sample rises with the Epoch Capabilities Index (Pearson $r=0.94$; microaveraged $r=0.95$). Each dot is one of the 61 of 66 judges Epoch scores. Hermes~3 405B, QwQ-32B-Preview, GLM-4.6, Qwen3.5~27B and Qwen3.8 2.4T-A95B have no score}{figure.caption.7}{}}
\externallabel{app:ty_ablations}{{E}{5}{}{appendix.E}{}}
\externallabel{app:ty_stability}{{E.1}{5}{}{subsection.E.1}{}}
\externallabel{fig:ty_stability}{{4}{6}{Accuracy varies little across five runs, and Q2 ideas and Q4 prose are the weakest cells in every run. Sol 6.1 flips more verdicts than Opus 5.5, and most of its flips cross between the human and AI sides of the five-level label rather than passing through \emph {mixed}. Top: mean accuracy (\%) on the 200-document stability set, with bars spanning the range across runs. Bottom: documents whose verdict changes in at least one run}{figure.caption.8}{}}
\externallabel{fig:ty_explain}{{5}{6}{Across five runs the explanations cite nearly the same evidence, and flipped verdicts differ only in secondary points. Each bar is the distribution of judge ratings of evidence overlap between the five explanations, from 1 (none) to 5 (identical); no rating is below 3, and the three 3s are too few to see. A verdict is flipped if it changes in at least one run}{figure.caption.9}{}}
\externallabel{app:ty_contamination}{{E.2}{7}{}{subsection.E.2}{}}
\externallabel{fig:ty_date_cue}{{6}{7}{A pre-LLM date in the explanation lowers Opus 5.5 accuracy on every AI-written dimension and on none of the human-written ones; the drop is largest on Q4 prose (80.3\% to 35.4\%), where the date belongs to the human source. Main-run accuracy (\%) with (filled) and without (open) a date cue}{figure.caption.10}{}}
\externallabel{tab:ty_fresh_set}{{6}{7}{Composition of the post-cutoff fiction set, 50 documents per quadrant. Opus 5.5 and Sol 6.1 each write 25 of the Q3 and Q4 stories, at xhigh effort and length-matched to the source story}{table.caption.11}{}}
\externallabel{fig:ty_fresh}{{7}{8}{Both detectors score the post-cutoff fiction set about as well as the main-run fiction evaluations, so contamination does not appear to inflate the fiction results. Filled: post-cutoff set (mean of five runs); open: main run}{figure.caption.12}{}}
\externallabel{app:ty_cutoff}{{E.3}{8}{}{subsection.E.3}{}}
\externallabel{fig:ty_score_dist}{{8}{9}{The scores of both detectors are bimodal, with few documents near the default cutoff of 0.5 (dashed). The cutoff giving 1\% FPR (dotted) is higher for Sol 6.1 than for Opus 5.5. Main-run \texttt {ai\_share} scores in bins of 0.05}{figure.caption.13}{}}
\externallabel{tab:ty_scores}{{7}{9}{Properties of the main-run \texttt {ai\_share} scores. Both detectors rank documents almost perfectly, but Sol 6.1 gives exactly 0 to about a quarter of documents while Opus 5.5 almost never does, and the cutoff for 1\% FPR differs by model. False-positive rates use the cleaned human documents (\S \ref {sec:method_data})}{table.caption.14}{}}
\externallabel{fig:ty_rules}{{9}{9}{A single cutoff fitted on the evaluation data improves on the default $\texttt {ai\_share}\geq 0.5$ by at most 2.8 points of balanced accuracy, and only per-source cutoffs gain more. Each point is the gain of one rule over the default, whose balanced accuracy is 94.0 and 96.1\% for Opus 5.5 and 93.5 and 96.7\% for Sol 6.1 (ideas and prose), on the main run without the stability documents. Ceilings are two-fold cross-fitted; Sol has no label rules because its main-run export has scores only}{figure.caption.15}{}}
\externallabel{fig:ty_q2_cutoff}{{10}{10}{Catching most Q2 ideas requires a cutoff near 0.15, which flags 22\% (Opus 5.5) and 34\% (Sol 6.1) of human-idea documents. Solid: Q2 documents flagged over the five stability runs; dashed: human-idea documents flagged in the main run; dotted: 0.5}{figure.caption.16}{}}
\externallabel{app:explanation-analysis}{{F}{10}{}{appendix.F}{}}
\externallabel{app:explanation-agreement}{{F.1}{10}{}{subsection.F.1}{}}
\externallabel{fig:explanation-annotation-interface}{{11}{12}{Human annotation interface for auditing explanation agreement. Annotators review grouped evidence items from two detector explanations, assess whether they share the same point, lean and reason, inspect unmatched items, and check the judge's proposed decisive-factor sets}{figure.caption.17}{}}
\externallabel{tab:manual-agreement}{{8}{12}{Human--human and Opus--human agreement on ideas and prose judgments. Annotator 1 completed 32 documents and Annotator 2 completed 24. Each score gives eligible documents equal weight. The decisive row uses candidate-membership AC1 and selected-set F1; other F1 rows compare positive labels}{table.caption.18}{}}
\externallabel{tab:manual-agreement-ideas}{{8}{12}{Human--human and Opus--human agreement on ideas and prose judgments. Annotator 1 completed 32 documents and Annotator 2 completed 24. Each score gives eligible documents equal weight. The decisive row uses candidate-membership AC1 and selected-set F1; other F1 rows compare positive labels}{table.caption.18}{}}
\externallabel{tab:manual-agreement-prose}{{8}{12}{Human--human and Opus--human agreement on ideas and prose judgments. Annotator 1 completed 32 documents and Annotator 2 completed 24. Each score gives eligible documents equal weight. The decisive row uses candidate-membership AC1 and selected-set F1; other F1 rows compare positive labels}{table.caption.18}{}}
\externallabel{fig:explanation-example}{{12}{13}{Example explanation (ideas part). An Opus 5.5 reply to the joint prompt for a human-written poem (MELD; fully human). Each evidence item gives a statement (\textbf {IDEA}), a lean, a strength, supporting quotes and a justification (\textbf {WHY}). The reply ends with a decisive factor and a verdict. When forming groups, the judge sees only the statements, quotes and decisive factor. For same reason, it sees the statements, leans and justifications. The prose part has the same form}{figure.caption.19}{}}
\externallabel{tab:explanation-agreement}{{9}{13}{\textbf {Opus 5.5 and GPT-6.1 Sol agree on verdicts more than on evidence, interpretation or decisive factor.} For each of 3{,}000 documents, an Opus 5.5 judge compares one saved Opus explanation with one saved Sol explanation (1{,}001 Q1, 1{,}000 Q3 and 999 Q4 documents spread over 25 datasets; Q2 has no further documents). \emph {Verdict}: both on the same side of $\texttt {ai\_share}=0.5$. \emph {Evidence F1}: the harmonic mean of $|\mathcal {G}|/(|\mathcal {G}|+|U_A|)$ and $|\mathcal {G}|/(|\mathcal {G}|+|U_B|)$, where $\mathcal {G}$ is the shared groups and $U_A,U_B$ are unmatched items. \emph {Interpretation}: share of shared points with the same lean and the same reason. \emph {Decisive F1}: $2|D_A\cap D_B|/(|D_A|+|D_B|)$ for the decisive sets of group IDs and unmatched decisive items, skipped when neither names a point (123 ideas pairs; 2{,}877 ideas documents scored). F1 is calculated per pair before averaging over documents; verdict and interpretation retain their original definitions and values. The Docs column gives the cohort size; decisive F1 uses its defined subset. Table~\ref {tab:stability-agreement} reports the 200-document stability study with the same F1 definitions. Judge outputs, not human-validated; Opus judges its own explanations}{table.caption.20}{}}
\externallabel{tab:opus-argon-agreement}{{10}{13}{\textbf {Opus 5.5 and Gemini 4 Argon also agree on verdicts more than on evidence, interpretation or decisive factor.} For each of 2{,}995 documents, the same Opus 5.5 judge, prompts and settings as in Table~\ref {tab:explanation-agreement} compare one saved Opus explanation with one saved Argon explanation (Argon at high thinking, from the main evaluation\textquoteright s batch run). These are the 3{,}000 documents of that table minus five that have no usable Argon explanation (four blocked by Gemini, one with unnumbered items); 997 Q1, 1{,}000 Q3 and 998 Q4 documents, spread over 25 datasets. Metrics, F1 averaging and exclusions are as in Table~\ref {tab:explanation-agreement}; decisive F1 skips 11 ideas pairs where neither decisive factor names a point. The Docs column gives the cohort size; decisive F1 uses its defined subset. Judge outputs, not human-validated; Opus judges its own explanations}{table.caption.21}{}}
\externallabel{tab:argon-sol-agreement}{{11}{14}{\textbf {Gemini 4 Argon and GPT-6.1 Sol also agree on verdicts more than on evidence, interpretation or decisive factor.} For each of 2{,}995 documents, the same Opus 5.5 judge, prompts and settings as in Table~\ref {tab:explanation-agreement} compare one saved Argon explanation with one saved Sol explanation (Argon at high thinking, from the main evaluation\textquoteright s batch run). These are the 3{,}000 documents of that table minus five that have no usable Argon explanation (four blocked by Gemini, one with unnumbered items); 997 Q1, 1{,}000 Q3 and 998 Q4 documents, spread over 25 datasets. Metrics, F1 averaging and exclusions are as in Table~\ref {tab:explanation-agreement}; decisive F1 skips 18 ideas pairs where neither decisive factor names a point. The Docs column gives the cohort size; decisive F1 uses its defined subset. Judge outputs, not human-validated on these pairs}{table.caption.22}{}}
\externallabel{tab:stability-agreement}{{12}{14}{Each model agrees with itself more than with the other model, at every level. Each model explained each of 200 documents five times with the same prompt. Within-model rows (Opus--Opus, Sol--Sol) score all 10 pairs of runs per document; the Opus--Sol row pairs run $k$ of Opus with run $k$ of Sol (5 pairs per document). Evidence and decisive overlap use the same per-pair F1 definitions as Table~\ref {tab:explanation-agreement}. Verdict and interpretation are unchanged. F1 is calculated for each pair before averaging defined pair scores within each document, then across documents with equal weight. Decisive is undefined for a pair when neither decisive factor names a point; the Decisive docs column counts documents with at least one defined pair. Judge outputs, not human-validated; Opus judges its own explanations}{table.caption.23}{}}
\externallabel{app:targeted-edits}{{F.2}{14}{}{subsection.F.2}{}}
\externallabel{tab:minjoon-agent:targeted-rq2}{{13}{15}{RQ2: changes in normalized developer/lab attribution relative to saved original predictions}{table.caption.24}{}}
\externallabel{tab:minjoon-agent:targeted-rq3}{{14}{16}{RQ3 Reddit pilot: predicted-username changes and original-source-author accuracy under Argon editing/detection}{table.caption.25}{}}
\externallabel{app:feat-analysis}{{F.3}{17}{}{subsection.F.3}{}}
\externallabel{app:feat-discovery}{{F.3.1}{17}{}{subsubsection.F.3.1}{}}
\externallabel{tab:cohort}{{15}{17}{Reason augmentation and feature coding on the main cohort. Each judge--target setup contains 2,432 document judgments}{table.caption.26}{}}
\externallabel{tab:catalogs}{{16}{17}{Final target-specific feature catalogs and their retained attribution directions}{table.caption.27}{}}
\externallabel{app:feat-assignment}{{F.3.2}{17}{}{subsubsection.F.3.2}{}}
\externallabel{tab:frequent-ideas}{{17}{18}{The ten most frequent ideas feature--attribution pairs for each judge, ranked by individual reason occurrences}{table.caption.28}{}}
\externallabel{tab:frequent-prose}{{18}{19}{The ten most frequent prose feature--attribution pairs for each judge, ranked by individual reason occurrences}{table.caption.29}{}}
\externallabel{app:minjoon-feature-agreement}{{F.3.3}{20}{}{subsubsection.F.3.3}{}}
\externallabel{tab:agreement}{{19}{20}{Opus--Sol verdict and feature agreement on the same 2,432 documents (all values in percent)}{table.caption.30}{}}
\externallabel{app:feat-verification}{{F.3.4}{20}{}{subsubsection.F.3.4}{}}
\externallabel{tab:prior}{{20}{21}{Selected examples of detector-cited features that align in meaning and attribution direction with prior findings}{table.caption.31}{}}
\externallabel{app:mk_multilingual}{{G}{21}{}{appendix.G}{}}
\externallabel{tab:mk_complete_coverage}{{21}{21}{Completed new-prompt dataset and judging coverage}{table.caption.32}{}}
\externallabel{tab:mk_complete_accuracy}{{22}{22}{Complete new-prompt family attribution accuracy by language, provenance and judgment}{table.caption.33}{}}
\externallabel{tab:mk_all_authors_en}{{23}{22}{English shared-provenance accuracy for all 19 author models}{table.caption.34}{}}
\externallabel{tab:mk_all_authors_non_en}{{24}{23}{non-English shared-provenance accuracy for all 19 author models}{table.caption.35}{}}
\externallabel{tab:mk_glm_versions}{{25}{23}{GLM version comparison on the same shared source briefs, using separate-family scoring}{table.caption.36}{}}
\externallabel{tab:mk_matched_accuracy_en}{{26}{24}{English matched old/new prompt accuracy}{table.caption.37}{}}
\externallabel{tab:mk_matched_accuracy_non_en}{{27}{24}{non-English matched old/new prompt accuracy}{table.caption.38}{}}
\externallabel{fig:mk_all_en_holistic_separate}{{13}{25}{English, shared provenance, holistic attribution under the new prompt. Families are separate. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.39}{}}
\externallabel{fig:mk_all_en_prose_separate}{{14}{26}{English, shared provenance, prose attribution under the new prompt. Families are separate. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.40}{}}
\externallabel{fig:mk_all_en_ideas_separate}{{15}{27}{English, shared provenance, ideas attribution under the new prompt. Families are separate. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.41}{}}
\externallabel{fig:mk_all_non_en_holistic_separate}{{16}{28}{non-English, shared provenance, holistic attribution under the new prompt. Families are separate. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.42}{}}
\externallabel{fig:mk_all_non_en_prose_separate}{{17}{29}{non-English, shared provenance, prose attribution under the new prompt. Families are separate. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.43}{}}
\externallabel{fig:mk_all_non_en_ideas_separate}{{18}{30}{non-English, shared provenance, ideas attribution under the new prompt. Families are separate. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.44}{}}
\externallabel{fig:mk_all_en_holistic_open_merged}{{19}{31}{English, shared provenance, holistic attribution under the new prompt. Open families are merged. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.45}{}}
\externallabel{fig:mk_all_en_prose_open_merged}{{20}{32}{English, shared provenance, prose attribution under the new prompt. Open families are merged. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.46}{}}
\externallabel{fig:mk_all_en_ideas_open_merged}{{21}{33}{English, shared provenance, ideas attribution under the new prompt. Open families are merged. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.47}{}}
\externallabel{fig:mk_all_non_en_holistic_open_merged}{{22}{34}{non-English, shared provenance, holistic attribution under the new prompt. Open families are merged. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.48}{}}
\externallabel{fig:mk_all_non_en_prose_open_merged}{{23}{35}{non-English, shared provenance, prose attribution under the new prompt. Open families are merged. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.49}{}}
\externallabel{fig:mk_all_non_en_ideas_open_merged}{{24}{36}{non-English, shared provenance, ideas attribution under the new prompt. Open families are merged. Rows distinguish all 19 author models; the first numeric column is family accuracy, and remaining cells are counts. Red-to-green accuracy colors have a fixed 0--100 percent scale. Blank cells are zero and green outlines mark correct-family cells}{figure.caption.50}{}}
\externallabel{fig:mk_mixed_new_en_mixed_ideas_separate}{{25}{38}{English, mixed provenance, ideas attribution under the new joint prompt. Families are separate. Rows distinguish the true idea-origin model or prose writer. Row sample sizes differ because same-family pairs are omitted. The first numeric column gives accuracy; other cells are counts}{figure.caption.51}{}}
\externallabel{fig:mk_mixed_new_en_mixed_ideas_open_merged}{{26}{38}{English, mixed provenance, ideas attribution under the new joint prompt. Open families are merged. Rows distinguish the true idea-origin model or prose writer. Row sample sizes differ because same-family pairs are omitted. The first numeric column gives accuracy; other cells are counts}{figure.caption.52}{}}
\externallabel{fig:mk_mixed_new_en_mixed_prose_separate}{{27}{39}{English, mixed provenance, prose attribution under the new joint prompt. Families are separate. Rows distinguish the true idea-origin model or prose writer. Row sample sizes differ because same-family pairs are omitted. The first numeric column gives accuracy; other cells are counts}{figure.caption.53}{}}
\externallabel{fig:mk_mixed_new_en_mixed_prose_open_merged}{{28}{39}{English, mixed provenance, prose attribution under the new joint prompt. Open families are merged. Rows distinguish the true idea-origin model or prose writer. Row sample sizes differ because same-family pairs are omitted. The first numeric column gives accuracy; other cells are counts}{figure.caption.54}{}}
\externallabel{fig:mk_mixed_new_non_en_mixed_ideas_separate}{{29}{40}{non-English, mixed provenance, ideas attribution under the new joint prompt. Families are separate. Rows distinguish the true idea-origin model or prose writer. Row sample sizes differ because same-family pairs are omitted. The first numeric column gives accuracy; other cells are counts}{figure.caption.55}{}}
\externallabel{fig:mk_mixed_new_non_en_mixed_ideas_open_merged}{{30}{40}{non-English, mixed provenance, ideas attribution under the new joint prompt. Open families are merged. Rows distinguish the true idea-origin model or prose writer. Row sample sizes differ because same-family pairs are omitted. The first numeric column gives accuracy; other cells are counts}{figure.caption.56}{}}
\externallabel{fig:mk_mixed_new_non_en_mixed_prose_separate}{{31}{41}{non-English, mixed provenance, prose attribution under the new joint prompt. Families are separate. Rows distinguish the true idea-origin model or prose writer. Row sample sizes differ because same-family pairs are omitted. The first numeric column gives accuracy; other cells are counts}{figure.caption.57}{}}
\externallabel{fig:mk_mixed_new_non_en_mixed_prose_open_merged}{{32}{41}{non-English, mixed provenance, prose attribution under the new joint prompt. Open families are merged. Rows distinguish the true idea-origin model or prose writer. Row sample sizes differ because same-family pairs are omitted. The first numeric column gives accuracy; other cells are counts}{figure.caption.58}{}}
\externallabel{fig:mk_matched_en_shared_holistic_separate}{{33}{43}{English, shared provenance, holistic attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.59}{}}
\externallabel{fig:mk_matched_en_shared_holistic_open_merged}{{34}{44}{English, shared provenance, holistic attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.60}{}}
\externallabel{fig:mk_matched_en_shared_ideas_separate}{{35}{45}{English, shared provenance, ideas attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.61}{}}
\externallabel{fig:mk_matched_en_shared_ideas_open_merged}{{36}{46}{English, shared provenance, ideas attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.62}{}}
\externallabel{fig:mk_matched_en_shared_prose_separate}{{37}{47}{English, shared provenance, prose attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.63}{}}
\externallabel{fig:mk_matched_en_shared_prose_open_merged}{{38}{48}{English, shared provenance, prose attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.64}{}}
\externallabel{fig:mk_matched_en_mixed_ideas_separate}{{39}{49}{English, mixed provenance, ideas attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.65}{}}
\externallabel{fig:mk_matched_en_mixed_ideas_open_merged}{{40}{50}{English, mixed provenance, ideas attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.66}{}}
\externallabel{fig:mk_matched_en_mixed_prose_separate}{{41}{51}{English, mixed provenance, prose attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.67}{}}
\externallabel{fig:mk_matched_en_mixed_prose_open_merged}{{42}{52}{English, mixed provenance, prose attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.68}{}}
\externallabel{fig:mk_matched_non_en_shared_holistic_separate}{{43}{53}{non-English, shared provenance, holistic attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.69}{}}
\externallabel{fig:mk_matched_non_en_shared_holistic_open_merged}{{44}{54}{non-English, shared provenance, holistic attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.70}{}}
\externallabel{fig:mk_matched_non_en_shared_ideas_separate}{{45}{55}{non-English, shared provenance, ideas attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.71}{}}
\externallabel{fig:mk_matched_non_en_shared_ideas_open_merged}{{46}{56}{non-English, shared provenance, ideas attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.72}{}}
\externallabel{fig:mk_matched_non_en_shared_prose_separate}{{47}{57}{non-English, shared provenance, prose attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.73}{}}
\externallabel{fig:mk_matched_non_en_shared_prose_open_merged}{{48}{58}{non-English, shared provenance, prose attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.74}{}}
\externallabel{fig:mk_matched_non_en_mixed_ideas_separate}{{49}{59}{non-English, mixed provenance, ideas attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.75}{}}
\externallabel{fig:mk_matched_non_en_mixed_ideas_open_merged}{{50}{60}{non-English, mixed provenance, ideas attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.76}{}}
\externallabel{fig:mk_matched_non_en_mixed_prose_separate}{{51}{61}{non-English, mixed provenance, prose attribution: old and new prompts on identical articles. Families are separate. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.77}{}}
\externallabel{fig:mk_matched_non_en_mixed_prose_open_merged}{{52}{62}{non-English, mixed provenance, prose attribution: old and new prompts on identical articles. Open families are merged. Row accuracy uses a fixed red-to-green 0--100 percent scale; prediction counts use blue, blank cells mean zero, and green outlines identify the correct family}{figure.caption.78}{}}
\externallabel{app:ai_vs_ai_full}{{H}{63}{}{appendix.H}{}}
\externallabel{app:ai_vs_ai_setup}{{H.1}{63}{}{subsection.H.1}{}}
\externallabel{tab:ai_vs_ai_writers}{{28}{63}{\textbf {Writing models.} The 32 models that write the stories, op-eds and news, by lab. Released: the date the model was first listed on OpenRouter. $^{*}$\,Version assumed from the op-ed alias (Gemini~3.8, Qwen Max) or texts written on the Gemini API rather than OpenRouter (Gemma~4 31B)}{table.caption.79}{}}
\externallabel{tab:ai_vs_ai_holistic}{{29}{64}{\textbf {Which model wrote it?} Four detectors, Opus~5.5, Gemini~4 Argon, GPT-6.1 Sol and DeepSeek~V4.1 Flash (DS, the 17 Oct release), each with the v8 holistic prompt at medium effort, on texts whose ideas and prose come from one model (shared provenance). Each of the 32 models writes in all three datasets: stories (the 25 shared StoryScope prompts, or the test32 and StoryScope originals for seven models), op-eds (Marzena's matched requests, in English) and news (Ty's 25 headlines). Each cell is the share of that model's texts (25 unless marked) for which the detector named the right lab (\%); darker is higher. Labs run from the best detected to the worst, newest model first}{table.caption.80}{}}
\externallabel{tab:ai_vs_ai_argon_levels}{{30}{64}{\textbf {Thinking longer does not help Argon.} Gemini~4 Argon with the v8 holistic prompt at thinking level medium and high, on the originals answered at both levels: right lab (\%, texts). Cost at batch prices for the run on the browser's 2,327 English originals, and mean output tokens per answer (thoughts included). At high, 10 answers hit the 32,768-token output cap and 2 were blocked}{table.caption.81}{}}
\externallabel{app:ai_vs_ai_all}{{H.2}{65}{}{subsection.H.2}{}}
\externallabel{app:ai_vs_ai_argon_levels}{{H.3}{65}{}{subsection.H.3}{}}
\externallabel{sec:md_mixed}{{H.4}{65}{}{subsection.H.4}{}}
\externallabel{tab:ai_vs_ai_joint}{{31}{65}{\textbf {Ideas and prose from different models.} Opus~5.5 with the v8 joint prompt, which names the model behind the ideas and, separately, the model behind the prose. Right lab (\%), prose / ideas, on originals (one model wrote both) and on rewrites of their IdeaLens outlines by another model (mixed provenance)}{table.caption.82}{}}
\externallabel{app:atrey_rq3}{{I}{65}{}{appendix.I}{}}
\externallabel{tab:atrey_rq3_full}{{32}{65}{RQ3 accuracy (\%, 95\% interval) by domain and judge. \emph {Matched}: texts first public after all four original judges' release dates (private reviews have no public date and are their own arm; papers and Reddit comments are all matched). \emph {Not AI}: texts Pangram~4.1 does not label AI\@. \emph {Carbon} (Gemini~4 Carbon, medium) replaces Argon: the same holistic prompts and texts through the Gemini Batch API, with the replies that hit the 32,768-token output cap rerun at 65,536 on the standard API (33 of the 87 stopped at 32,768 again and stay out of the denominator). Carbon was not run on the original Reddit condition. Additional rows add the 36 later private reviews by a sixth writer (\emph {with sixth writer}: all 398 private reviews) and the 70 Nature-family reviews, whose publication dates are unverified, so they have only an \emph {all} view. Neither set was run with Qwen or has a not-AI row. Papers, Opus: 41/118 is 34.7\%; 34.8 comes from rounding an already rounded value. \emph {Fable 5.2} (Claude Fable 5.2, high effort): Atrey's OpenRouter batch run on the frozen texts (Reddit with the username prompt, as for the other judges), plus a run on the 36 later private reviews and the 70 Nature-family reviews with the same prompt and route; 7 of the 70 Nature-family reviews were refused}{table.caption.83}{}}
\externallabel{tab:atrey_rq3_reddit}{{33}{66}{RQ3 Reddit: accuracy (\%) with the exact-username prompt, by the author's activity in the comment's subreddit (Opus answered 47, 559, 250, 217, 164 comments per bin), and overall with the original full-name prompt, scored against the same usernames. The two prompt conditions are separate runs on the same 1,258 comments. \emph {Carbon} (Gemini~4 Carbon, medium) replaces Argon: the same holistic prompts and texts through the Gemini Batch API, with the replies that hit the 32,768-token output cap rerun at 65,536 on the standard API (33 of the 87 stopped at 32,768 again and stay out of the denominator). Carbon was not run on the original Reddit condition}{table.caption.84}{}}
\externallabel{tab:atrey_rq3_private}{{34}{66}{RQ3 private reviews by contributor (anonymised, ordered by number of reviews): accuracy (\%). Five people wrote the 362 reviews, so the texts are not independent. F, is a sixth writer whose 36 reviews were added later, so F is listed last; with F, six people wrote the 398 private reviews. Qwen was not run on F's reviews. The Fable 5.2 column is in blue, from the same runs as in \autoref {tab:atrey_rq3_full}. \emph {Carbon} (Gemini~4 Carbon, medium) replaces Argon: the same holistic prompts and texts through the Gemini Batch API, with the replies that hit the 32,768-token output cap rerun at 65,536 on the standard API (33 of the 87 stopped at 32,768 again and stay out of the denominator). Carbon was not run on the original Reddit condition}{table.caption.85}{}}
\externallabel{tab:atrey_rq3_pangram}{{35}{66}{RQ3 accuracy (\%) by the Pangram~4.1 label of the exact judged text. Texts labelled AI are almost never attributed. \emph {Carbon} (Gemini~4 Carbon, medium) replaces Argon: the same holistic prompts and texts through the Gemini Batch API, with the replies that hit the 32,768-token output cap rerun at 65,536 on the standard API (33 of the 87 stopped at 32,768 again and stay out of the denominator). Carbon was not run on the original Reddit condition}{table.caption.86}{}}
\externallabel{tab:atrey_rq3_cost}{{36}{66}{RQ3 inference cost across the three runs (API usage at list or batch rates, and Qwen's GPU allocation including failed time); estimates, not invoices. Carbon is its later run (Batch rates, and standard rates for the reruns at the higher output cap); Argon stays listed because its joint-prompt, familiarity and agreement results are still reported}{table.caption.87}{}}
\externallabel{app:atrey_rq3_deep}{{J}{67}{}{appendix.J}{}}
\externallabel{app:atrey_familiarity}{{J.1}{67}{}{subsection.J.1}{}}
\externallabel{tab:atrey_rq3_familiarity}{{37}{67}{RQ3 accuracy (\%, correct/answered) by whether the judge says it knows the writer. Holistic prompt, all selected texts; Reddit uses the username prompt. Opus gave familiarity ratings on Reddit separately, per account (below)}{table.caption.88}{}}
\externallabel{app:atrey_floors}{{J.2}{67}{}{subsection.J.2}{}}
\externallabel{tab:atrey_rq3_floors}{{38}{68}{RQ3 chance floors and writer clustering on the matched set (private reviews: all). Accuracy and floor in \%. Fable 5.2 rows use the same rules on Atrey\textquotesingle s batch run; its bootstrap and one-per-writer draws use their own random seed. Carbon (Gemini~4 Carbon, medium) replaces Argon, with the same texts, prompt and rules}{table.caption.89}{}}
\externallabel{app:atrey_clues}{{J.3}{68}{}{subsection.J.3}{}}
\externallabel{tab:atrey_rq3_slices}{{39}{68}{RQ3 public reviews by slice: accuracy (\%, correct/answered). Citation counts come from OpenAlex for the reviewers uniquely linked in an earlier study, so only part of the set is covered. Slices overlap and are not causal effects. Fable 5.2: Atrey\textquotesingle s batch run, same rules. Carbon (Gemini~4 Carbon, medium) replaces Argon, with the same texts, prompt and rules}{table.caption.90}{}}
\externallabel{app:atrey_release}{{J.4}{69}{}{subsection.J.4}{}}
\externallabel{tab:atrey_rq3_release}{{40}{69}{RQ3 stories first public before and after each judge\textquotesingle s release, within fame tier (\%, correct/answered). Named authors are found about as often in text the judge cannot have seen, so memorising the text does not explain the result. Cells are small}{table.caption.91}{}}
\externallabel{app:atrey_consensus}{{J.5}{69}{}{subsection.J.5}{}}
\externallabel{tab:atrey_rq3_consensus}{{41}{69}{RQ3 agreement. Same name: texts where Opus and Argon give one person, of those where both name someone; \ldots {} right: how often that person is the writer (\%). Any of three and all three: Opus, Argon and Sol (\%)}{table.caption.92}{}}
\externallabel{app:atrey_conf}{{J.6}{69}{}{subsection.J.6}{}}
\externallabel{tab:atrey_rq3_conf}{{42}{69}{Joint prompt: share of texts (\%) where the judge is more confident in its ideas answer than in its prose answer, and the reverse; the rest are ties}{table.caption.93}{}}
\externallabel{tab:deniz-agent:rq3-joint-accuracy}{{43}{70}{RQ3 accuracy (\%) under the holistic prompt and for the two answers of the joint prompt, on the matched texts (36 stories, 120 papers, 218 public reviews, 362 private reviews, 1,258 Reddit comments). Accuracy is over answered texts. Public and Private are peer reviews; Reddit uses the username prompt}{table.caption.94}{}}
\externallabel{tab:deniz-agent:rq3-joint-same-author}{{44}{70}{Joint prompt: texts (\%) where the ideas answer and the prose answer name the same person, after name normalisation, over all texts with two valid answers (not only the matched texts); two answers that both name nobody count as the same. Reddit here uses the full-name prompt, on which Argon was not run, so Argon\textquotesingle s All excludes Reddit. All pools texts across domains}{table.caption.95}{}}
\externallabel{app:deniz-agent:rq3-agreement-rerun}{{J.7}{70}{}{subsection.J.7}{}}
\externallabel{tab:deniz-agent:rq3-blind-agreement}{{45}{71}{Condition-blind RQ3 explanation agreement on original texts. Stability scores average pairs within document before averaging documents; cross-model scores average one pair per document. The stability and cross-model samples differ. Pairs are valid matches; decisive F1 excludes both-empty decisive sets}{table.caption.96}{}}
\externallabel{tab:deniz-agent:icml-review-agreement}{{46}{71}{ICML 2020 review agreements. Mean pair-level F1 for condition-blind matches of holistic explanations. Same-review comparisons use different models; the other conditions use one model across distinct reviews. Same predicted author uses normalized named predictions and does not require them to be correct. One mixed-model judge response is excluded}{table.caption.97}{}}
\externallabel{app:deniz-agent:rq3-rewrite-agreement}{{J.8}{71}{}{subsection.J.8}{}}
\externallabel{tab:deniz-agent:rq3-rewrite-agreement}{{47}{72}{Original versus first rewrite: mean explanation overlap F1 from the current blind 1,000-document study. Each cell is mean F1 (number of documents with a defined score). Overall means weight scored documents equally, not domains equally; they are not population-weighted. Validation exclusions differ between models, and both-empty decisive sets are excluded separately. Public-review sampling follows the source preparation rather than the later strict cohort; Nature-family reviews are not included}{table.caption.98}{}}
\externallabel{app:deniz-agent:rq3-author-repeat-stability}{{J.9}{72}{}{subsection.J.9}{}}
\externallabel{tab:deniz-agent:rq3-three-run-author-agreement}{{48}{72}{Agreement in the attributed author across three independent judgments on the same text. Counts are documents. Missing or recognized abstaining answers are excluded from the three-answer categories. Opus had six missing or refused original judgments}{table.caption.99}{}}
\externallabel{tab:deniz-agent:rq3-correct-to-wrong}{{49}{72}{Correct-to-wrong changes across repeats. Among documents whose original judgment was correct, the last two columns count documents with at least one wrong repeat and with both repeats wrong. One originally correct Opus judgment had a missing or abstaining repeat, which is not counted as wrong. Correctness uses the RQ3 author and username matching rules, including any listed paper coauthor}{table.caption.100}{}}
\externallabel{tab:deniz-agent:rq3-rewrite-accuracy}{{50}{73}{Attribution accuracy before and after rewriting on the RQ3 matched cohort. Columns: the original text, the first Argon rewrite (Rew.~1) and a second independent Argon rewrite (Rew.~2) of the same source, all judged by Argon or Opus~5.5 with the same holistic prompt. Cells give percent correct over the $n$ texts with a valid judgment of all three versions, the same texts in every column within a judge. Reddit asks for the exact username; a paper counts as correct when any listed author is named; reviews and stories use the shared RQ3 full-name rule}{table.caption.101}{}}
\externallabel{app:deniz-agent:rq3-rewrite-accuracy}{{J.10}{73}{}{subsection.J.10}{}}
\externallabel{app:deniz-agent:rq3-fame-tiers}{{J.11}{73}{}{subsection.J.11}{}}
\externallabel{fig:deniz-agent:rq3-fame-tiers}{{53}{73}{Earlier version of \autoref {fig:rq3_fame}, with story authors sorted into four fame tiers instead of Goodreads ratings. T1: a household name, roughly 10 or more books with major bestsellers; T2: an established author with 3 or more books and a bestseller, prize or adaptation; T3 and T4: lesser-known writers. Pilot authors were tiered by hand and the rest by a proxy from Wikipedia page views, Wikimedia sitelinks and Open Library work counts. Correct/answered stories, T1 to T4: Fable~5.2 29/29, 32/32, 29/62, 6/121; Opus~5.5 26/29, 24/32, 13/62, 1/121; Argon 26/29, 25/32, 9/61, 1/119; Sol 26/29, 27/32, 17/62, 2/121}{figure.caption.102}{}}
\externallabel{app:atrey_claude_refusals}{{K}{73}{}{appendix.K}{}}
\externallabel{tab:atrey_claude_refusals}{{51}{74}{Recorded Claude refusals by cohort and execution route. Counts are per request, including refusals in the denominator; the two joint judgments share one request. ICML counts use the saved export\textquotesingle s refusal classification. The other rows use saved refusal flags, outcomes or refusal stops; these do not exhaust text-only refusals. CLI denotes Claude Code. The fiction timeline has one refusal (Fable~5.1); Opus~4.6 has only 82 saved fiction responses, giving 1,161 requests in total. Unknown-author answers and other errors are separate. Cohorts and settings differ, so the table does not identify a causal CLI/API effect}{table.caption.103}{}}
\externallabel{app:prompts}{{L}{74}{}{appendix.L}{}}
\externallabel{app:prompt_holistic}{{L.1}{74}{}{subsection.L.1}{}}
\externallabel{app:prompt_joint}{{L.2}{74}{}{subsection.L.2}{}}
\externallabel{app:prompt_rq3_holistic}{{L.3}{75}{}{subsection.L.3}{}}
\externallabel{app:prompt_rq3_joint}{{L.4}{76}{}{subsection.L.4}{}}
\externallabel{app:prompt_rq3_reddit}{{L.5}{77}{}{subsection.L.5}{}}
\externallabel{app:prompt_familiarity}{{L.6}{77}{}{subsection.L.6}{}}
\makeatother


==> tables/captions.tex <==
\newcommand{\capLLM}{GPT-6.1 Sol and Claude Opus 5.5 are gpt-6.1-sol and claude-opus-5-5 with one joint prompt; the cell is the accuracy of their ideas verdict, flagged at an ai\_share of at least 0.5 (no calibrated cut), on a sample of at most 663 documents per arm. The in-domain ladders were not run (--).}
\newcommand{\capCons}{\textbf{Every detector, every quadrant.} Each cell is the mean over evaluations of the evaluation's pooled rate in that quadrant, at the global 1\% cut (own thresholds for the detectors marked own). Q1: human ideas, human prose; Q4: human ideas, model prose; Q3: model ideas, model prose, with the attacked and humanized arms as a separate column; Q2: model ideas, human prose. A superscript gives the number of evaluations where a detector covers fewer than the column's total. A provenance detector is low in Q1 and Q4 and high in Q3 and Q2; a surface detector rises in Q4 and falls in Q2. \capLLM{}}

\newcommand{\capAblations}{\textbf{In-domain results and ablations} for the two outline-trained models. Top: the held-out test split. Middle: the same models read a transformed outline, with the 1\% cut refitted on the transformed calibration split; the roles-only row also gives a separately trained roles-only \mb{}. Bottom: the share of verdicts that survive paraphrasing, sentence-level paraphrase of the source and a change of extractor, and the cost of reading a 500-word excerpt.}

\newcommand{\capMultiling}{\textbf{\xLadder{}, selected languages (\%).} FineWeb2 pages in each language (human: false-positive rate), a
model writing natively in that language from one line naming the document type and broad subject (level 0: TPR), and a model rendering the page's outline in that language with nothing
added (level 5: false-positive rate under the provenance rule). \model{} reads English outlines extracted from every language; it has never
seen a non-English document. Global 1\% cut for our models, Pangram~4 at its published threshold. All 24 languages in \S\ref{app:multiling}.}

\newcommand{\capProbe}{\textbf{Paraphrasing removes most of the surface signal.} Pangram~4 scores 1,000 held-out test documents three ways: as the document, the raw outline, and the paraphrased outline. We report the mean and median (shaded) of Pangram's human, AI-assisted, and AI fractions and of P(AI) $=$ AI $+\,\frac{1}{2}$ AI-assisted, in percent. On paraphrased outlines, Pangram rates almost every human document as AI, while \model{} still separates them. AUC is against the Pangram~3.3.2 labels, so the document row is partly circular.}

\newcommand{\capQone}{\textbf{Human ideas, human prose: accuracy (\%).} Ordinary human writing, so accuracy is the share labeled human. The top two rows give each detector's mean accuracy in this quadrant and in the other three, so no detector can look strong by always predicting one label. Outline column: global 1\% cut\,/\,per-format cut. $^{\dagger}$All documents under 500 words. All arms are in \S\ref{app:evals}. \capLLM{}}

\newcommand{\capQfour}{\textbf{Human ideas, model prose: accuracy (\%).} A model wrote, rewrote, or polished a person's content, so accuracy is the share labeled human. The top two rows give each detector's mean accuracy in this quadrant and in the other three, so no detector can look strong by always predicting one label. Outline column: global 1\% cut\,/\,per-format cut. $^{\dagger}$All documents under 500 words. All arms are in \S\ref{app:evals}. \capLLM{}}

\newcommand{\capQthree}{\textbf{Model ideas, model prose: accuracy (\%).} Conventional machine-text detection; accuracy is TPR, and attacked or humanized arms are marked. PeerPrism \citep{peerprism} and the personal-style set \citep{baumler-etal-2026-make} are left out (\S\ref{app:benchmarks}). $^{\dagger}$every document under 500 words. Every arm of every evaluation is in \S\ref{app:evals}. \capLLM{}}

\newcommand{\capQtwo}{\textbf{Model ideas, human prose: accuracy (\%).} People wrote \aiipset{} in their own words from a model's stories; accuracy is TPR. The other sets in this quadrant, where a person edited or polished a model's text rather than rewriting it, are in \S\ref{app:q2full}.  $^{\dagger}$every document under 500 words. Every arm of every evaluation is in \S\ref{app:evals}. \capLLM{}}

\newcommand{\capMixed}{\textbf{Mixed authorship is a gradation, not a rate.} Mean P(AI) (\%; median in parentheses where reported) for arms where a model wrote from a person's ideas or a person from a model's (shaded), shown between their evaluation's clear model-idea and human-idea arms. These arms are not counted in any quadrant table. Pangram~4's P(AI) is AI $+\,\frac{1}{2}$ AI-assisted. All levels, with minima and maxima, are in \S\ref{app:evals}.}

\newcommand{\capExtractBench}{\textbf{Outline extraction benchmark.} Twelve extractors on 198 documents, scored against Claude Fable 5 reference outlines. We report (a) order-preserving match of outline items (\emph{alignment}) (b) reference/candidate items matched (\emph{coverage}) (c) one-to-one matches (\emph{granularity agreement}) (d) candidate minus reference items per match (\emph{split$-$merge}) (e) exact label match (\emph{role agreement}) (f) cost per document with batching (g) mean rank (1 is best) and mean score from GPT-5.6 Sol, which judges eight configurations per document against the reference without seeing their source; a cross-check on the alignment score (``--'': not judged). Corpus extractors are in bold.
}

\newcommand{\capSolQuad}{\textbf{GPT-6.1 Sol and the detectors by quadrant: accuracy (\%).} Share of documents labeled correctly against the quadrant's prose label (prose columns) or idea label (idea columns), averaged over the evaluations with arms in the quadrant (Evals). Sol counts a document as model-made when \texttt{ai\_share} is at least 0.5; \twinmodel{} reads the document and \model{} the outline, both at the global 1\% cut. Documents are a subsample of each evaluation (\S\ref{app:sol_protocol}). \twicetold{}'s \model{} figures are the counts in \S\ref{sec:results}.}

\newcommand{\capSolEvals}{\textbf{GPT-6.1 Sol and the detectors, by evaluation: balanced accuracy (\%).} Mean of the true positive rate and one minus the false positive rate, on documents both models scored; ``--'' means the evaluation has only one class for that question. The last two rows pool all documents and average over the evaluations that have both classes.}

\newcommand{\capSolArms}{\textbf{GPT-6.1 Sol and the detectors, every arm: share flagged as model-made (\%).} Rows with a human label are false positive rates, rows with a model label are true positive rates, and arms with a human-leaning or model-leaning idea label are fire rates. $n$ is the number of documents. $^{\dagger}$\twicetold{}'s \model{} figures are the counts reported in \S\ref{sec:results}; per-story flags are not available.}

\newcommand{\capSolMl}{\textbf{\xLadder{} trial: share flagged as model-made (\%) by language resource group.} Nine languages (three per group), 30 sources each, with the human page, level 0 (model ideas, model prose) and level 5 (human ideas, model prose) for each source. Groups follow FineWeb2 size (\S\ref{app:evals}). GPT-6.1 Sol reads English prompts and English outlines; \twinmodel{} reads the document and \model{} the outline.}

\newcommand{\capFrontQuad}{\textbf{GPT-6.1 Sol and Claude Opus 5.5 against the detectors, by quadrant: accuracy (\%).} One joint prompt asks each model, from the document, who came up with the ideas and who wrote the prose; a document is flagged as model-made when the model's \texttt{ai\_share} is at least 0.5. Idea detection is scored against the ideas label and prose detection against the prose label, so a flag is right where the label is model and wrong where it is human. Cells are means over all evaluations of each evaluation's accuracy on the pooled arms of the quadrant, including the appendix-only evaluations, so they differ slightly from the means in the main tables; the attacked and humanized arms are separate rows. \model{} and \twinmodel{} are at their global 1\% cuts and Pangram~4 at its published threshold (the weighted rule used in the other tables); the last two columns are Pangram~4's own verdict, counting ``mixed'' as model-made or not. Sol and Opus~5.5 score a sample of at most 663 documents per arm, the detectors every document; the ladders and the resource-tier arms are not run. \twicetold{} has 50 stories. Instances is the number scored for Sol (Opus~5.5 scored 144 fewer, which it declined).}

\newcommand{\capFrontArms}{\textbf{GPT-6.1 Sol and Claude Opus 5.5, every arm: accuracy (\%).} Same protocol as \autoref{tab:frontier_quad}. $n$ is the number of documents scored for Sol. Accuracy is the catch rate where the label is model and one minus the false-alarm rate where it is human.}


==> tables/minjoon-agent_attribution_examples.tex <==
\begin{table*}[!t]
\centering\footnotesize
\definecolor{cueTeal}{HTML}{437E8E}\definecolor{cueTealBg}{HTML}{E3EFF2}\definecolor{cueClay}{HTML}{B4501C}\definecolor{cueClayBg}{HTML}{FBEDE4}\definecolor{cueRose}{HTML}{6E2042}\definecolor{cueRoseBg}{HTML}{FBEBF1}
\newcommand{\exmark}[2]{{\setlength{\fboxsep}{0pt}\colorbox{#1Bg}{\textcolor{#1}{\strut #2}}}}
\caption[Claude Fable 5.2 examples]{\protect\iconFable\,Claude Fable~5.2 bases each decision on concrete evidence ranging from mixed apostrophes to a reviewer's self-description. Each explanation lists quoted evidence and names decisive factors. In each row, a \exmark{cueRose}{highlighted} reason shares its color with the words in the text it describes.}
\label{tab:attribution-examples}
\vspace{6pt}
\begingroup
\definecolor{predictionCorrect}{HTML}{00AB89}
\newcommand{\predlabel}[1]{{\fontsize{5.5}{7}\selectfont\MakeUppercase{#1}}}
\newcommand{\predtag}[1]{{\setlength{\fboxsep}{1.6pt}\mbox{\colorbox{black!9}{\rule{0pt}{6.6pt}\textbf{#1}}\,\textcolor{predictionCorrect}{\ensuremath{\checkmark}}}}}
\newcommand{\predmeta}[1]{{\scriptsize #1}}
\setlength{\tabcolsep}{2pt}\renewcommand{\arraystretch}{1.05}
\begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash\hyphenpenalty=10000}p{.132\linewidth}>{\raggedright\arraybackslash}p{.30\linewidth}>{\raggedright\arraybackslash}p{.165\linewidth}>{\raggedright\arraybackslash}X@{}}
\toprule
\textbf{Task} & \textbf{Text (excerpt)} & \textbf{\iconFable\,Prediction} & \textbf{\iconFable\,Explanation (excerpt)} \\
\midrule
\textbf{Human or AI?}\par Story from TwiceTold: \textit{lantern and firefly} & ``\exmark{cueRose}{The }\allowbreak \exmark{cueRose}{most }\allowbreak \exmark{cueRose}{meaningful }\allowbreak \exmark{cueRose}{light }\allowbreak \exmark{cueRose}{is }\allowbreak \exmark{cueRose}{that }\allowbreak \exmark{cueRose}{which }\allowbreak \exmark{cueRose}{is }\allowbreak \exmark{cueRose}{provided }\allowbreak \exmark{cueRose}{in }\allowbreak \exmark{cueRose}{moments }\allowbreak \exmark{cueRose}{of }\allowbreak \exmark{cueRose}{need.} [\ldots] \exmark{cueTeal}{From }\allowbreak \exmark{cueTeal}{that }\allowbreak \exmark{cueTeal}{day }\allowbreak \exmark{cueTeal}{on,} travelers to the forest always saw two lights [\ldots] the lantern never again \exmark{cueClay}{mistook }\allowbreak \exmark{cueClay}{greatness }\allowbreak \exmark{cueClay}{with }\allowbreak \exmark{cueClay}{size}.'' & \predlabel{Ideas}\par\predtag{AI}\ \predmeta{90\% AI}\par\vspace{4pt}\predlabel{Prose}\par\predtag{Human}\ \predmeta{10\% AI} & \textbf{Ideas:} ``The deciding factor is the concentration of stock choices: [\ldots] and the \exmark{cueRose}{stated }\allowbreak \exmark{cueRose}{moral} with a \exmark{cueTeal}{"from }\allowbreak \exmark{cueTeal}{that }\allowbreak \exmark{cueTeal}{day }\allowbreak \exmark{cueTeal}{on" }\allowbreak \exmark{cueTeal}{coda}.''\par\smallskip \textbf{Prose:} ``The deciding factors are the \exmark{cueClay}{non-idiomatic }\allowbreak \exmark{cueClay}{and }\allowbreak \exmark{cueClay}{ungrammatical }\allowbreak \exmark{cueClay}{slips: }\allowbreak \exmark{cueClay}{"mistook }\allowbreak \exmark{cueClay}{greatness }\allowbreak \exmark{cueClay}{with }\allowbreak \exmark{cueClay}{size"}'' \\
\addlinespace[2.5pt]
\textbf{Which AI?}\par AI story from \textit{StoryScope} & ``Luke \exmark{cueTeal}{didn\textquotesingle{}t} hesitate. [\ldots] He looked at \exmark{cueTeal}{Harry\textquoteright{}s} trembling shoulders. [\ldots] \exmark{cueRose}{The }\allowbreak \exmark{cueRose}{Gulf }\allowbreak \exmark{cueRose}{was }\allowbreak \exmark{cueRose}{a }\allowbreak \exmark{cueRose}{graveyard, }\allowbreak \exmark{cueRose}{but }\allowbreak \exmark{cueRose}{for }\allowbreak \exmark{cueRose}{tonight, }\allowbreak \exmark{cueRose}{the }\allowbreak \exmark{cueRose}{brothers }\allowbreak \exmark{cueRose}{were }\allowbreak \exmark{cueRose}{still }\allowbreak \exmark{cueRose}{ghosts }\allowbreak \exmark{cueRose}{in }\allowbreak \exmark{cueRose}{the }\allowbreak \exmark{cueRose}{making, }\allowbreak \exmark{cueRose}{drifting }\allowbreak \exmark{cueRose}{on }\allowbreak \exmark{cueRose}{the }\allowbreak \exmark{cueRose}{tide }\allowbreak \exmark{cueRose}{of }\allowbreak \exmark{cueRose}{a }\allowbreak \exmark{cueRose}{dying }\allowbreak \exmark{cueRose}{world.} [\ldots] \exmark{cueRose}{Row. }\allowbreak \exmark{cueRose}{Steer. }\allowbreak \exmark{cueRose}{Live. }\allowbreak \exmark{cueRose}{And }\allowbreak \exmark{cueRose}{never, }\allowbreak \exmark{cueRose}{ever }\allowbreak \exmark{cueRose}{laugh.}'' & \predlabel{Model}\par\predtag{Gemini 3 Flash}\par\vspace{3pt}\predlabel{Developer}\par\predtag{Google}\par\vspace{3pt}\predmeta{Confidence 40\%} & ``The deciding factor is the combination of the \exmark{cueRose}{stacked, }\allowbreak \exmark{cueRose}{aphoristic }\allowbreak \exmark{cueRose}{endings }\allowbreak \exmark{cueRose}{with }\allowbreak \exmark{cueRose}{a }\allowbreak \exmark{cueRose}{staccato }\allowbreak \exmark{cueRose}{coda} and the \exmark{cueTeal}{mixed }\allowbreak \exmark{cueTeal}{curly }\allowbreak \exmark{cueTeal}{and }\allowbreak \exmark{cueTeal}{straight }\allowbreak \exmark{cueTeal}{apostrophes} with trailing spaces. The stylistic habits alone could fit several models, but the formatting artifacts are much more specific to Gemini [\ldots] The specific version remains a best guess.'' \\
\addlinespace[2.5pt]
\textbf{Which human?}\par Review from \textit{Nature Sustainability} & ``\exmark{cueRose}{I }\allowbreak \exmark{cueRose}{am }\allowbreak \exmark{cueRose}{primarily }\allowbreak \exmark{cueRose}{a }\allowbreak \exmark{cueRose}{wellbeing }\allowbreak \exmark{cueRose}{researcher} [\ldots] \exmark{cueClay}{emphasises} [\ldots] \exmark{cueClay}{what }\allowbreak \exmark{cueClay}{matters }\allowbreak \exmark{cueClay}{for }\allowbreak \exmark{cueClay}{policy }\allowbreak \exmark{cueClay}{seems }\allowbreak \exmark{cueClay}{rather }\allowbreak \exmark{cueClay}{to }\allowbreak \exmark{cueClay}{be }\allowbreak \exmark{cueClay}{any }\allowbreak \exmark{cueClay}{substantive }\allowbreak \exmark{cueClay}{magnitudes }\allowbreak \exmark{cueClay}{of }\allowbreak \exmark{cueClay}{any }\allowbreak \exmark{cueClay}{relationships.} [\ldots] \exmark{cueTeal}{between }\allowbreak \exmark{cueTeal}{long-run }\allowbreak \exmark{cueTeal}{changes }\allowbreak \exmark{cueTeal}{in }\allowbreak \exmark{cueTeal}{GDP }\allowbreak \exmark{cueTeal}{per }\allowbreak \exmark{cueTeal}{capita }\allowbreak \exmark{cueTeal}{and }\allowbreak \exmark{cueTeal}{long-run }\allowbreak \exmark{cueTeal}{changes }\allowbreak \exmark{cueTeal}{in }\allowbreak \exmark{cueTeal}{wellbeing}'' & \predlabel{Reviewer}\par\predtag{Caspar Kaiser}\par\vspace{3pt}\predmeta{Confidence 27\%} & ``The deciding factor is the combination of three things: the \exmark{cueRose}{self-description }\allowbreak \exmark{cueRose}{as }\allowbreak \exmark{cueRose}{"primarily }\allowbreak \exmark{cueRose}{a }\allowbreak \exmark{cueRose}{wellbeing }\allowbreak \exmark{cueRose}{researcher"}, the \exmark{cueTeal}{specialist }\allowbreak \exmark{cueTeal}{long-run }\allowbreak \exmark{cueTeal}{reading }\allowbreak \exmark{cueTeal}{of }\allowbreak \exmark{cueTeal}{the }\allowbreak \exmark{cueTeal}{Easterlin }\allowbreak \exmark{cueTeal}{Paradox}, and \exmark{cueClay}{UK-style }\allowbreak \exmark{cueClay}{orthography }\allowbreak \exmark{cueClay}{with }\allowbreak \exmark{cueClay}{faintly }\allowbreak \exmark{cueClay}{non-native }\allowbreak \exmark{cueClay}{syntax}. The Easterlin point narrows the field to a few specialists, and the spelling and phrasing eliminate most of the others.'' \\
\addlinespace[2.5pt]
\textbf{Which human?}\par Human story: \textit{Lost Child} & ``\exmark{cueTeal}{For}, with Kit\textquoteright{}s father, something was always either going to happen or had already happened, [\ldots] \exmark{cueClay}{Hurry, }\allowbreak \exmark{cueClay}{sweetie! }\allowbreak \exmark{cueClay}{God }\allowbreak \exmark{cueClay}{damn.} \exmark{cueRose}{Not }\allowbreak \exmark{cueRose}{used }\allowbreak \exmark{cueRose}{to }\allowbreak \exmark{cueRose}{dressing }\allowbreak \exmark{cueRose}{herself.} [\ldots] but maybe Daddy wouldn\textquoteright{}t notice.'' & \predlabel{Author}\par\predtag{\shortstack[l]{Joyce Carol\\Oates}}\par\vspace{3pt}\predmeta{Confidence 93\%} & ``The deciding factor is the combination of style and theme: \exmark{cueRose}{fragmentary, }\allowbreak \exmark{cueRose}{subject-dropping }\allowbreak \exmark{cueRose}{sentences}, \exmark{cueTeal}{sentence-initial }\allowbreak \exmark{cueTeal}{"For"}, and \exmark{cueClay}{unquoted }\allowbreak \exmark{cueClay}{menacing }\allowbreak \exmark{cueClay}{speech}, [\ldots] this particular pairing of syntax and subject matter is characteristic of Oates and outweighs the generic literary-fiction features.'' \\
\bottomrule
\end{tabularx}
\endgroup
\end{table*}

